Multimodal Approaches to Fair Image Classification: An Ethical Perspective

In the rapidly advancing field of artificial intelligence, machine perception is becoming paramount to achieving increased performance. Image classification systems are becoming increasingly integral to various applications, ranging from medical diagnostics to image generation; however, these systems often exhibit harmful biases that can lead to unfair and discriminatory outcomes. Machine Learning systems that depend on a single data modality, i.e. only images or only text, can exaggerate hidden biases present in the training data, if the data is not carefully balanced and filtered. Even so, these models can still harm underrepresented populations when used in improper contexts, such as when government agencies reinforce racial bias using predictive policing. This thesis explores the intersection of technology and ethics in the development of fair image classification models. Specifically, I focus on improving fairness and methods of using multiple modalities to combat harmful demographic bias. Integrating multimodal approaches, which combine visual data with additional modalities such as text and metadata, allows this work to enhance the fairness and accuracy of image classification systems. The study critically examines existing biases in image datasets and classification algorithms, proposes innovative methods for mitigating these biases, and evaluates the ethical implications of deploying such systems in real-world scenarios. Through comprehensive experimentation and analysis, the thesis demonstrates how multimodal techniques can contribute to more equitable and ethical AI solutions, ultimately advocating for responsible AI practices that prioritize fairness.

==> 00-titlepages.tex <==
%% Replace all of the orange portions with your personal info

\begin{titlepage}
\begin{center}
\vspace*{\fill}
\singlespace
\thispagestyle{empty}
{\LARGE { \thesisTitle \\} %self-explanatory
\doublespacing
\vspace*{\baselineskip}
{\large \authorName }\\ %self-explanatory
\vspace*{1.5\baselineskip}
\large A dissertation
\\ submitted in partial fulfillment of the\\
requirements for the degree of\\
\vspace*{\baselineskip}
Doctor of Philosophy\\
\vspace{1.5\baselineskip}
University of Washington
\\ \graduationYear}\\ % add year in YYYY format (e.g. 2020)
\vspace{1.5\baselineskip}

%add reading committee (just the reading committee, not the supervisory committee):
\large \textit{Reading Committee:} \\

\ifdefined\secondAdvisor 
    \advisor, Co-Chair \\
    \secondAdvisor, Co-Chair \\
\else
    \advisor, Chair
\fi

\readingCommitteeOne \\

\ifdefined\readingCommitteeTwo
    \readingCommitteeTwo \\
\fi
    

\vspace{2\baselineskip}
  Program Authorized to Offer Degree: \\
Computer Science and Engineering
  
% \newcommand{\advisor}{Main Guardian}
% % if you have two advisors, uncomment these two
% \newcommand{\firstAdvisor}{Parent One}
% \newcommand{\secondAdvisor}{Parent Two}
% \newcommand{\readingCommitteeOne}{First Reader}
% \newcommand{\readingCommitteeTwo}{Second Reader}

  
  
%%% Insert year and name:
  \vspace*{\fill}
  \clearpage
  \thispagestyle{empty}
  \singlespace{
  \copyright~Copyright \graduationYear \\ %add year in YYYY format (e.g. 2020)
  \vspace*{\baselineskip}
  \authorName} %self-explanatory
\end{center}
\end{titlepage}


